Identifying and Analyzing Sepsis States: A Retrospective Study on Patients with Sepsis in ICUs

Sepsis accounts for more than 50% of hospital deaths, and the associated cost ranks the highest among hospital admissions in the US. Improved understanding of disease states, severity, and clinical markers has the potential to significantly improve patient outcomes and reduce cost. We develop a computational framework that identifies disease states in sepsis using clinical variables and samples in the MIMIC-III database. We identify six distinct patient states in sepsis, each associated with different manifestations of organ dysfunction. We find that patients in different sepsis states are statistically significantly composed of distinct populations with disparate demographic and comorbidity profiles. Collectively, our framework provides a holistic view of sepsis, and our findings provide the basis for future development of clinical trials and therapeutic strategies for sepsis.

==> methods.tex <==
\subsection*{Patient cohort.}


\textcolor{black}{We use the sepsis cohort defined by AI Clinician \cite{komorowski2018artificial}. Patient samples were collected from five distinct ICUs in Boston, Massachusetts, stored in the Medical Information Mart for Intensive Care version III (MIMIC-III) database. Patients that are diagnosed with sepsis when they had both suspicion of infection, defined as the presence of the prescription of antibiotics and sampling of bodily fluids for microbiological culture (as also used in prior work of Nemati et al. \cite{nemati2018interpretable}, Johnson et al. \cite{johnson2018comparative}, and recommended by the Sepsis-3 criteria \cite{singer2016third}), and the evidence of organ dysfunction, defined as the total SOFA score higher than 2 (baseline SOFA scores are assumed to be zero.\cite{seymour2016assessment, raith2017prognostic}), within the time window of 48 hours before and up to 24 hours after onset of infection. As recommended by the Sepsis-3 criteria \cite{singer2016third}, the time of the onset is defined as the earliest event of the following two conditions: i) if the antibiotic was given first, the microbiological sample must have been collected within 24 hours; ii) if the microbiological sampling occurred first, the antibiotic must have been administered within 72 hours. Finally, sepsis patients whose age was less than 18 years old at the time of ICU admission, whose mortality was not documented, and withdrawal of treatment (vasopressors) were excluded from our cohort.}

\subsection*{Data preprocessing.}
\textcolor{black}{Data were included from up to 24 hours prior to the estimated onset of sepsis and 48 hours after the onset to capture the characteristics of the early stages of sepsis. \textcolor{black}{The resulting cohort includes 16,546 distinct patients with 20,944 stays in ICUs.} Patients’ data are modeled as discrete multivariate time series with 4-hour time steps. Clinical variables associated with the patients are demographics, vital signs, lab values, severity measures such as SIRS and SOFA scores, and other information relating to use of ventilator and the number of comorbidities before sepsis infection. We also track whether the patient survived for 48 hours and extract the history of 30 types of comorbidities \cite{elixhauser1998comorbidity} before infection, as supplementary variables. Outliers were removed when the clinical variables were out of normal range (e.g., weight larger than 300 kg and blood pressure below 0). If there are multiple measurements within the 4 hour time period, either the max values are taken (e.g., vasopressor), are averaged (e.g., heart rate), or are accumulated (e.g., urine output and fluids). To address the issue of missing values,  we use time-limited sample-and-hold method \cite{hug2009detecting} for each variable with a different maximum hold time to identify missing values. Linear interpolation and k-nearest-neighbor methods were then used for the imputations \cite{tutz2015improved}.   }


\subsection*{Archetypal analysis.\cite{cutler1994archetypal}}
\label{sec:arch_analysis_formulation}

Archetypal analysis views each point in a dataset as a mixture (convex combination) of ``pure types'', or ``archetypes''. The convexity constraint here implies that in contrast to traditional clustering techniques that aim to identify ``typical'' representatives, archetypal analysis aims to identify ``extremal'' points in the dataset. The archetypes  are themselves mixtures (convex combinations) of the points in the data set. Archetypes can be learned by minimizing the squared error in representing each point as a mixture of archetypes. Specifically, let $\xx_{1},\dots,\xx_{n}$ be the data points in $\mathcal{R}^m$. The problem is to find a set of archetypes $\{\zz_{1},\dots,\zz_{K}\}$ so that each archetype $\zz_k$ is a convex combination of the data points, \textit{i.e.,} $\sum^n_{j=1} \beta_{kj}\xx_j$, with the constraints of: (i)  $\beta_{kj} \geq 0 \quad \forall j $; and (ii)      $\sum^n_{j=1}\beta_{kj}=1$ (convexity constraint), and that each data point $\xx_i$ can be best approximated by a convex combination of the archetypes, \textit{i.e.}, $\sum^K_{k=1}\alpha_{ik}\zz_k$, with the constraints: (i) $\alpha_{ik} \geq 0 \quad \forall i$; and (ii) $\sum^p_{k=1}\alpha_{ik}=1$. 

We can then define the following optimization problem: 
\begin{align}
    \min_{\{\alpha_{ik},\beta_{kj}\}}\sum^n_{i=1} \norm{\xx_i - \sum^p_{k=1}\alpha_{ik}\sum^n_{j=1}\beta_{kj}\xx_j }^2 \label{eq:AA_obj},
\end{align}
and the archetype problem is to find $\alpha$'s and $\beta$'s to minimize the objective \ref{eq:AA_obj} subject to the aforementioned constraints. This problem can be solved using general-purpose constrained nonlinear least squares methods, the alternating minimizing algorithm, or the projected gradient procedure. The learned archetypes (for $K$ >1) form a convex hull of the data set such that all of the points can be well-represented as a convex mixture of the archetypes. In our study, we first treat patient measurements as points in a high-dimensional space, and find archetypes for our cohort. These archetypes represent extreme states in sepsis, and each patient can be expressed as a convex combination of these states. We also use archetypal analysis to identify the archetypes of the transitions of clinical measurements. Please see Section \ref{sec:transition} for a detailed discussion.



\subsection*{Testing statistical significance of states.}\label{sec:significant-testing}

We characterize the statistical significance of each sepsis state based on the data points (patient records) mapped to the corresponding archetype from the cohort. Each point is a mixture of sepsis states, and we can assign the point to the closest sepsis state (the corresponding archetype). 
A statistical interpretation of this formulation views data points as mixtures of samples from the six distinct multivariate distributions. To ascertain that these distributions are indeed distinct, we first validate that the probability distributions corresponding to these groups are significantly different from the distribution of the cohort as a whole. We also test to ensure that the probability distribution of each group is significantly different from others, as characterized by a multivariate analysis of variance (MANOVA) procedure. Two-sample testing is sensitive to the homogeneity of covariance matrices from the compared populations. We use the Box test to compare variation in multivariate samples. We then use a Hotelling T-Squared testing variant to compare the mean vectors from two populations. We note that covariance matrices and mean vectors from the compared pairs are significantly different, with a 95 \% confidence interval. \textcolor{black}{Statistics of pairwise Hotelling t-square test across sepsis states and two-sample t-test for each variable for each sepsis state are shown in Table \ref{fig:t2-test} and Table \ref{fig:t-test}, respectively.} 

\subsubsection*{Comparing mean vectors from two populations.}

We use Two-sample Hotelling's T$^2$ tests to characterize significant differences between the mean vectors of two multivariate distributions (in reality, datasets drawn from these distributions). Two-sample Hotelling's T$^2$ tests are sensitive to violations of the assumption of equal variances and covariances. Different approximation of the sample variance is needed when the covariance matrices of the two populations are significantly different. We use Box’s M test for significant differences between covariance matrices.


\paragraph{Testing homogeneity of covariance matrices : Box’s M Test.}

Consider a sample set $\{\xx_{11},\dots,\xx_{1n_1}\}$ in $\mathcal{R}^m$ sampled from population $\Theta_1$ and a sample set $\{\xx_{21},\dots,\xx_{2n_2}\}$ in $\mathcal{R}^m$ sampled from population $\Theta_2$. Assuming that the sample sizes $n_1$ and $n_2$ are sufficiently large, Box’s M Test tests the null hypothesis that the population covariance matrices are equal, \textit{i.e.}, $H_0 : \Sigma_1=\Sigma_2$. Let $S_1$ and $S_2$ be the sample covariance matrices from the populations $\Theta_1$ and $\Theta_2$, where each $S_j$ is based on $n_j$ independent observations, we define the pool variance $S_{pooled}$ as follows:
\begin{align*}
    &S_{pooled} = \frac{1}{n_1+n_2-2} (n_1-1)S_1 +(n_2 -1)S_2,\\
\end{align*}
and the value of $M$ is given by:
\begin{align*}
    &M = (n_1+n_2 -2)\ln|S_{pooled}| - \left( (n_1 -1)\ln|S_1| +(n_2-1)\ln|S_2| \right).
\end{align*}
Then, $M(1-c)$  has an approximate $\chi^2_{df}$-distribution, where: 
%
\begin{align*}
    & c= \frac{2m^2+3m-1}{6(m+1)(n_1+n_2-1)}\left( 
    \frac{1}{n_1-1}+\frac{1}{n_2-1}-\frac{2}{n_1+n_2-2}\right),\\
    & df= \frac{m(m+1)(n_1+n_2-1)}{2}.
\end{align*}
The null hypothesis $H_0$ is rejected when $M(1 - c ) > \chi^2_{df}(\alpha)$ (or p-value < $\alpha$) .


\paragraph{Testing homogeneity of mean vectors : Hotelling’s T-Squared test.}

We test the equality of vector means from populations $\Theta_1$ and $\Theta_2$. The null hypothesis is that the population means are equal, \textit{i.e.,} $H_0 : \boldsymbol{\mu_1}=\boldsymbol{\mu_2}$. If Box’s M test indicates that the two covariance matrices are not significantly different, we can assume $\Sigma_1=\Sigma_2$ and:
\begin{align*}
    &T^2 = (\bar{\xx}_1-\bar{\xx}_2)^\intercal \left( (\frac{1}{n_1+n_2}) S_{pooled} \right)^{-1}(\bar{\xx}_1-\bar{\xx}_2).\\
\end{align*} 
If Box’s M test concludes that $\Sigma_1 \neq \Sigma_2$, 
\begin{align*}
    &T^2 = (\bar{\xx}_1-\bar{\xx}_2)^\intercal \left( \frac{1}{n_1}S_1 + \frac{1}{n_2}S_2\right)^{-1}(\bar{\xx}_1-\bar{\xx}_2)
\end{align*}
In either case, $T^2$ approximates chi-square distribution with $m$ degrees of freedom, \textit{i.e.,} $\chi^2_{m}$. The null hypothesis is rejected when $T^2> \chi^2_{m}(\alpha)$ (or p-value < $\alpha$) .


\subsection*{Low-dimensional embeddings of dataset.}

We use Uniform Manifold Approximation and Projection (UMAP)\cite{mcinnes2018umap} to compute a mapping from a dataset $X=\{\xx_1,\dots,\xx_n\}$ in $\mathcal{R}^m$ to its corresponding lower-dimensional representation $Y=\{\yy_1,\dots,\yy_n\}$ in $\mathcal{R}^d$ that preserves as much of the local and the global structure from the original space. UMAP assumes that the dataset $X$ is uniformly drawn from a Riemannian manifold $M$. With this assumption, the goal is to reconstruct $M$ and to find a mapping from $M$ into $\mathcal{R}^d$. To do so, UMAP first approximates the manifold and finds a  fuzzy simplicial set that captures all topological properties of the manifold $M$. Similarly, given a current lower-dimensional representation in $Y'$ of the data $X$ in $\mathcal{R}^m$, it can also construct a fuzzy simplicial set from $Y'$. Having the two fuzzy simplicial sets, one constructed from $X$ and the other constructed from $Y'$, UMAP then measures how good $Y'$ is as a representation of $X$ using cross-entropy $C$ of two fuzzy sets:
\begin{align*}
    C( (A,\mu),(A,\upsilon)) = \sum_{a\in A} \left(\mu(a)\log(\frac{\mu(a)}{\upsilon(a)}) + (1-\mu(a))\log(\frac{1-\mu(a)}{1-\upsilon(a)}) \right)
\end{align*}

The above objective function can be minimized using first-order optimization methods or second-order methods\cite{kylasa2020parallel,fang2018newton}.
%Once the objective is minimized, the corresponding solution $Y'$ is close to $Y$.

\subsection*{Feature selection methods.\cite{dudek2007cluster}}\label{sec:feature-selection}

\textcolor{black}{
Three criteria are developed to identify discriminative attributes for each state. The first method, which we refer to as the $Q_j(P_K)$, calculates the discriminative power of feature $i$ for a given clustering as the ratio of inter-cluster inertia to the total inertia computed using feature $i$. Intuitively, this method quantifies the heterogeneity of feature $i$ across clusters. The second method, which we refer to as $Q'_j(P_K)$, calculates the discriminative power of feature $i$ as the ratio of inter-cluster inertia computed using attribute $i$ to total inter-cluster inertia computed using all attributes. Intuitively, this method computes the relative heterogeneity of feature $i$ with respect to all other features. The third method uses a variation test that selects features with the lowest probability of overlap across clusters.}
\subsubsection*{Quality-index based approach.}

%{\bf ayg: can you clean the following paragraph? Are $x$'s the weights or $w$s the weights? If $x$s are the weights (as it would appear from the sentence following "Define ....", they what are $w$s?}
%\textcolor{black}{chf: just editted directly.}


Given a set $S = \{\xx_{1},\dots, \xx_{N}\}$ of $N$ points in $\mathcal{R}^m$ that is partitioned as $P_K= \{C_1,\dots,C_K \}$, where for each cluster pair $C_i, C_j$ $, 1\leq i,j,\leq K$ and $i\neq j$, $C_i\bigcap C_j = \Phi$, define $\bgg_k$ to be the mean values of the instances in cluster $C_k$, $\bgg$ be the average values over all the instances in $S$, the total inertia $T = \sum^N_{i=1} d^2(\xx_i,\bgg)
$ measures the dispersion of the points in the set $S$, where $d^2(\xx_i,\xx_{i'}) = \sum^m_{j=1} (x_{ij}-x_{i'j})^2 $ is the squared Euclidean distance. According to Huygens-Steiner Theorem, the total inertia $T$ can be decomposed into inter-cluster inertia $B$ and within-cluster inertia $W$:
\begin{align*}
    T &= B+W \\
       &= \sum^K_{k=1} d^2(\bgg_k,\bgg) + \sum^K_{k=1} I(C_k)\\
       &= \sum^K_{k=1} d^2(\bgg_k,\bgg) + \sum^K_{k=1}\sum_{i\in C_k} d^2(\xx_i,\bgg_k)
\end{align*}
Here, inter-cluster inertia $B$ measures the separation between the clusters, $I(C_k)$ is the inertia for cluster $C_k$, and the within-cluster inertia $W$ is the summation of the inertia of the clusters that measures the heterogeneity within the clusters.


\iffalse
\paragraph*{Quality Index.}
The quality index the ratio of the homogeneity value of each cluster and the corresponding homogeneity value associated with the partition $P_0 = S$, \textit{i.e.,} the entire dataset. This can be interpreted as the gap between the null hypothesis, \textit{i.e.,} partition into one cluster, and the given partition in $k$ clusters.

\paragraph{Partition Quality.} Given a set of points $S$ and a partition $P_k$, the null hypothesis is the total inertia $T$. Since the total inertia is a constant, the smaller the within-cluster inertia $W$, the larger the inter-cluster inertia $B$. The optimal strategy of assigning clusters is to minimize the inertia for each cluster. This leads to the following ratio as a measure of partition quality: 

\begin{align*}
    Q(P_k)=\frac{B}{T} = 1- \frac{W}{T}= 1 - \frac{I(W)}{I(T)}.
\end{align*}

\fi

\paragraph{Variable quality.} The \textit{quality index} is given by the ratio of the homogeneity value of each cluster and the corresponding homogeneity value associated with the partition $P_0 = S$. This can be interpreted as the gap between the null hypothesis, \textit{i.e.,} partition into one cluster, and partition into $k$ clusters. We can use the quality index at each variable (in our case, patient feature) $j$ to find the importance of the features.  Given a set of points $S$ partitioned by $P_K$, the null hypothesis is that the total inertia of the system is $T_j$. Since the partition $P_K$ is given, the total inertia of the system is fixed at $T_j$ and the optimal strategy of assigning clusters is to select minimal within-cluster inertia, $W_j$. This leads to the following ratio as a measure of variable quality: 
%
\iffalse
We can also define a quality measure in the variable level to compute the contribution of each variable  into the resulting clusters. Similar to the partition quality $Q(P_k)$, the variable quality can be defined as: 
\fi
%
\begin{align*}
    &Q_j(P_k)=\frac{B_j}{T_j} = 1- \frac{W_j}{T_j},\\
    &W_j= \sum_{i\in C_k} (x_{ij}-g_{kj})^2,\\
    &T_j= \sum^N_{i=1} (x_{ij}-g_j)^2.
\end{align*}
%
%
Alternatively, since the partition $P_K$ is given, we can ignore the variability of within-cluster inertia in the variable quality measure. That is, we only consider how each variable contributes to the total  inter-cluster inertia:
\begin{align*}
    &Q'_j(P_k)=\frac{B_j}{\sum^p_{i=1}B_i}.
\end{align*}

In our study, we use both  $Q_j(P_K)$ and $Q'_j(P_K)$ variable quality measures for feature selection. We also include a third feature selection criteria based on a variation test.


\subsubsection*{Variation test.}

Given a partition $P_K=\{C_1,\dots,C_K\}$ of a set of points $S$, we can regard the points in cluster $C_i$ as being sampled from a distinct multivariate probability distribution $\Theta_i$. To find the $j$-th feature that can distinguish the clusters, there exist at least two pairs of marginal distributions such that the difference of the mean value at the $j$-th feature sampled from the compared marginal distributions is larger than some threshold $\theta$ with probability $1-\delta$, where $\delta$ is sufficiently small.  We set $\theta=\sigma_{ij}$ when comparing clusters $C_i$ and $C_l$ ($l \neq i$) and collect the union of the variables from each case as the selected features. Although this feature selection method treats each dimension independently, we find that the selected features are similar to those using quality-index based approaches. See section supplementary \ref{sec:feature_sel} for a detailed comparison.




\subsection*{Expression of primary functions.} \label{sec:primary_function_expression}

\textcolor{black}{
 We measure the overall expression of each of these primary functions for each sepsis state, shown as a  spider-plot of primary functions affected in each sepsis state in Figure \ref{fig:primary_function}, using the level of corresponding biomarkers, weighted by the confidence level (as measured by the number of overlaps between feature selection methods). For sepsis state $i$, we calculate the distance $d_i$ between readings from the biomarkers to the boundary of the normal range for each primary function. We then normalize each $d_i$ by dividing  by the maximum of the distance across sepsis states, \textit{i.e.}, $d_i/\max\{d_1,\dots,d_K\}$. Since each primary function can be tested by more than one biomarker, each of which has a different confidence level, we define the final expression of the primary function as a summation of normalized distances. The final value is linearly normalized into the range from 0 to 10, with higher values indicating higher expression of primary function. }



%{\bf ayg: I cant understand the next paragraph.. the percentage of what? can you please restate these and I'll edit again?}

%\textcolor{black}{We have developed feature selection methods to find the most prominent features by measuring (i) the ratio of between-cluster inertia at the i-th feature $B_i$ to the total inertia at the i-th feature $T_i$, (ii) the ratio of the between-cluster inertia at i-th feature $B_i$ to the total between-cluster inertia $\sum^p_{i=1}B_i$ ,  (iii) and the feature that has a lower probability of overlapping between clusters.}

\iffalse
\subsubsection*{Confidence ranking algorithm.} 

%We use feature selection methods for quantifying: (i) the percentage of between-cluster at the i-th feature inertia is of the total inertia at the i-th feature, (ii) the percentage of the between-cluster inertia at i-th feature is of the total between-cluster inertia,  (iii) and the feature that has a lower probability of overlapping between clusters. 

Although there is a considerable overlap among selected features between the three feature selection methods, there are few features that are uniquely selected based on each of the selection criteria. We use a  confidence ranking algorithm, shown in \ref{alg-ranking}, to quantify our confidence in associating a feature with an archetype. 

%for the selected features with time complexity $\mathcal{O}(lm)$, where $l$ and $m$ denotes the number of feature selection methods and the dimensionality of the samples respectively.

\begin{algorithm} [!htbp]
\caption{Feature Confidence Ranking Algorithm}\label{alg-ranking}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Results}{Results}
	\Input{  \\
		$\{L_1,\dots,L_l \} $ - a set of l lists of selected variables collected from m selecting methods  \\
			 }
	\Results{\\
	        $Rank\_Dict$ - a dictionary of the rankings for the selected variables.
			}
	\For{ $i = 1,\dots, m$ }		{ \For{ $ j = 1, \dots, m $ }{ 
		\If{ $L_j$ is not empty }{
			$ele = L_j.pop()$\\
            \eIf{$Rank\_Dict.get(ele)$ is None}{
                $Rank\_Dict(ele)=1;$
            }{
            $Rank\_Dict(ele)=Rank\_Dict(ele)+1;$
            }
		}
		}
	}
   \Return{$Rank\_Dict;$}

\end{algorithm}

\paragraph{Runtime analysis for confidence ranking algorithm ~\ref{alg-ranking}.}
The outer loop in Algorithm ~\ref{alg-ranking} executes $l$ times, and the inner loop, $m$ times. In each iteration, the algorithm checks whether a list is empty, retrieves an element from a list, checks if a key exists in the dictionary, and updates the value of the corresponding key-value pairs in the dictionary. These operations can be done in $\mathcal{O}(1)$ time. The overall time complexity of the algorithm is $\mathcal{O}(lm)$.

\fi

\iffalse
Ok. Given K clusters, each one of cardinality $n_k$ such that the sum of the $n_k$'s returns N the cardinality of the instances, described by P features, the
$BET_{SSQ}=\sum_{k=1,..,K} n_k \sum_{p=1,...,P} (m_{k,p}-m_{p})^2$,
where $m_{k,p}$ is the mean of the feature p in the cluster k and $m_p$ the mean of the feature p over all the instances.
The
$WIT_{SSQ}=\sum_{i=1,...,N}\sum(p=1,...,P) \sum_{k=1,...,K} I(i,k)(x_{i,p}-m_{k,p})^2$
where I(i,k)=1 if the i-th instance belongs to the k-th cluster, 0 otherwise, and $x_{i,p}$ is the value of the i-th instance for the feature p.
Finally the $TOTAL_{SSQ}=\sum_{i=1,...,N}\sum(p=1,...,P)(x_{i,p}-m_{p})^2$
and it is easy to prove that $TOTAL_{SSQ}=BET_{SSQ}+WIT_{SSQ}$, it is also known with the name of Huygens decomposition of the inertia. Indeed, $TOTAL_SSQ$ is known also as Total inertia of a set of points around its center.
Naturally the same decomposition holds for each feature, i.e.
$TOTAL_{SSQ}(p)=BET_{SSQ}(p)+WIT_{SSQ}(p)=
\sum_{k=1,..,K} n_k (m_{k,p}-m_{p})^2+\sum_{i=1,...,N}\sum_{k=1,...,K} I(i,k)(x_{i,p}-m_{k,p})^2.
$


\fi



\textcolor{black}{\subsection*{Z-score analysis for comorbidity profiles.} We assess whether the comorbidity profile of interest is uniquely expressed or suppressed in a certain sepsis state. We compute the corresponding Z-score:}
\begin{align*}
    \textcolor{black}{z^i_{j} = \frac{w^i_{j}-\mu_j}{\sigma_j},}
\end{align*} 
\textcolor{black}{where $\mu_j$ is the rate of presence of comorbidity $j$ among all the patients in the cohort, $\sigma_j$ is its corresponding standard deviation, and $w^i_{j}$ is the reference point, calculated as the rate of the presence of comorbidity $i$ among patients who have passed through sepsis state $j$. Here, $z^i_{j}$ measures how far the reference point $w^i_{j}$ is from the population mean for the sepsis state $i$. If $z^i_{j}$ is positive, $w^i_{j}$ is expressed in sepsis state $i$, and vice versa.}


\subsection*{Analysis of Sepsis progression.}

\paragraph{Higher-order Markov chains.}
\label{sec:markov_chain}

Higher-order Markov chains are used to model transitions across sepsis states \cite{raftery1985model}. Formally, given a dataset (observational traces) $\mathcal{D}$ from m patients.
\begin{align*}
    \mathcal{D}&\triangleq \Big\{ \{\textbf{h}_i =  \{(t_{ij},\xx_{ij},a_{ij})\}_{j=1}^{n_i}  \Big\}_{i=1}^{m} \\ 
&= \left\{\begin{array}{lr}
        \textbf{h}_1=\{(t_{1j},\xx_{1j},a_{1j})\}_{j=1}^{n_1}\\
         \quad\quad\quad\quad\quad \vdots\\
        \textbf{h}_m=\{(t_{mj},\xx_{mj},a_{mj})\}_{j=1}^{n_m}
        \end{array}\right\} 
\end{align*} 
where $\textbf{h}_i$ denotes patient $i$'s \textit{trace} with $n_i$ time ordered points, and each point is defined as $(t,\xx,a)$, meaning that at time $t$, clinical measurements $\xx$, and sepsis state $a$ are observed. We model the transition of disease through these states using a higher-order Markov chain. The transition probability of $l$-th order Markov model can be written as:
\begin{align*}
  \Pr[\mathcal{S}_t=i_0|\mathcal{S}_{t-1}=i_1,\dots,\mathcal{S}_{t-1}=i_l] ,
\end{align*} where $l \geq 1$ denotes the order of a Markov chain and $i_j$ denotes the realization of sepsis state at time point $t-j$. The higher-order Markov model can be represented as a directed valued De Bruijn graph, denoted as $\mathcal{B}(K,l)$, where the set of vertices is given by:
\begin{align*}
  V = \mathcal{A}^K=\{(a_1,\dots,a_1,a_1),(a_1,\dots,a_1,a_2),\dots,(a_1,\dots,a_1,a_K),(a_1,\dots,a_2,a_1),\dots,(a_K,\dots,a_K,a_K)\},
\end{align*}
and the set of edges is given by:
\begin{align*}
  E=\{((\hat{a}_1,\hat{a}_2,\dots,\hat{a}_l),(\hat{a}_2,\dots,\hat{a}_l,a_j)): a_i \in \mathcal{A}, 1\leq i \leq l , 1\leq j\leq K\},
\end{align*} where each edge takes the value of its corresponding transition probability.  In our study, we analyze sepsis transitions up to third order Markov models.

\paragraph{Identification of transition markers.}
\label{sec:transition}

Archetypal analysis and z-score analysis are used to identify transition markers across sepsis states. Formally, let transition dataset $\mathcal{G}=\{g_1,\dots,g_{m'}\}$ represent gradients of clinical measurements on transition from one sepsis state to another, collected from dataset $\mathcal{D}$ of $m$ patients. We first find distinct groupings of gradients using archetypal analysis. That is, given a transition dataset $\mathcal{G}=\{g_1,\dots,g_{m'}\}$, we aim to find a set of archetypes of gradients so that each gradient is a convex combination of archetypes and each archetype is a convex combination of the gradients. Once archetypes are identified, we define gradient states by mapping the gradient points to the corresponding archetype. We then compute z-scores to find the transition markers by finding the subset of features (components) of each cluster that are over-represented or suppressed. The z-score is computed as follows:
\begin{align*}
    z^{i}_{j} = \frac{\mu^{i}_{j}-\bar{\mu_j}}{\bar{\sigma_j}}.
\end{align*} 
Here, $\bar{\mu_j}$ is the mean value of $j$-th feature over the entire population, $\bar{\sigma_j}$ is its corresponding standard deviation, and $\mu^{i}_{j}$ is the mean value of $j$-th feature for gradient group $i$. The z-score $z^{i}_{j}$ measures how far the reference point $\mu^{i}_{j}$ is from the population mean for the gradient group $i$. If $z^{i}_{j}$ is positive, $\mu^{i}_{j}$ is expressed in gradient group $i$, and vice versa.

